Deciphering the unusual stellar progenitor of GRB 210704A

GRB~210704A is a burst of intermediate duration ($T_{90} \sim 1-4$~s) followed by a fading afterglow and an optical excess that peaked about 7 days after the explosion. Its properties, and in particular those of the excess, do not easily fit into the well established classification scheme of GRBs as being long or short, leaving the nature of its progenitor uncertain. We present multi-wavelength observations of the GRB and its counterpart, observed up to 160 days after the burst. In order to decipher the nature of the progenitor system, we present a detailed analysis of the GRB high-energy properties (duration, spectral lag, and Amati correlation), its environment, and late-time optical excess. We discuss three possible scenarios: a neutron star merger, a collapsing massive star, and an atypical explosion possibly hosted in a cluster of galaxies. We find that traditional kilonova and supernova models do not match well the properties of the optical excess, leaving us with the intriguing suggestion that this event was an exotic high-energy merger.

==> GRB 210704A/galaxies.tex <==
S1  & 159.0201 & 57.2163 & $2.15 \pm 0.10$ & 25.20 $\pm$ 0.20 & 0.19 $\pm$ 0.14 & 14.86 $\pm$ 11.17 & 0.02 & 0.40 \\
S2  & 159.0205 & 57.2157 & - & 24.68 $\pm$ 0.08 & 2.36 $\pm$ 0.12 & - & 0.12 & 0.40 \\
G1 & 159.0179 & 57.2243 & 0.0817 & 16.23 $\pm$ 0.00 & 29.28 $\pm$ 0.09 & 52.26 $\pm$ 0.17 & 0.005 & 2.39 \\
%G2 & 159.0045 & 57.20661 & 0.17 & 17.55 $\pm$ 0.01 & 46.34 $\pm$ 0.09 & 181.84 $\pm$ 0.37 & 0.06 & 2.39 \\
%G3 & 159.0477 & 57.22218 & 0.20 & 18.31 $\pm$ 0.01 & 57.62 $\pm$ 0.09 & 268.94 $\pm$ 0.44 & 0.22\footnote{The chance probability is much lower ($\approx$0.001) if one considers the association between the GRB and the galaxies' cluster hosting G3.} & 1.52 \\


==> GRB 210704A/observations.tex <==
0.38 & 360& \emph{ w }& $>$ 19.70 & DDOTI & \cite{30383}, This work \\
0.73 & 3038& \emph{ v }& $>$ 21.10 & UVOT/SWIFT & \cite{30389} \\
0.94 & 3960& \emph{ r' }& 22.25 $\pm$ 0.13 & AZT-20 & \cite{30384} \\
1.08 & 1560& \emph{ r }& 22.13 $\pm$ 0.13 & DOLORES/TNG & \cite{30385} \\
1.08 & 900& \emph{ z' }& $>$ 21.50 & OAJ-T80 & \cite{30401} \\
1.09 & 900& \emph{ i' }& 22.08 $\pm$ 0.23 & OAJ-T80 & \cite{30401} \\
1.09 & 1500& \emph{ i' }& 21.84 $\pm$ 0.13 & CAFOS/CAHA & \cite{30391} \\
1.09 & 120& \emph{ r }& 22.40 $\pm$ 0.07 & OSIRIS/GTC & \cite{30392} \\
1.10 & 900& \emph{ g' }& 22.42 $\pm$ 0.11 & OAJ-T80 & \cite{30401} \\
1.12 & 900& \emph{ r' }& 22.17 $\pm$ 0.10 & OAJ-T80 & \cite{30401} \\
1.29 & 1152& \emph{ i }& $>$ 22.10 & RATIR & \cite{30390} \\
1.29 & 1152& \emph{ r }& $>$ 22.40 & RATIR & \cite{30390} \\
2.07 & 27000& \emph{ r }& $>$ 22.70 & CAFOS/CAHA & \cite{30411} \\
2.10 & 420& \emph{ r }& 23.43 $\pm$ 0.11 & OSIRIS/GTC & This work \\% (Alan 2022-03-13) \\
2.10 & 420& \emph{ z }& 23.44 $\pm$ 0.30 & OSIRIS/GTC & This work \\%(Alan 2022-03-13)\\
3.92 & 4620& \emph{ r' }& $>$ 23.10 & AZT-20 & \cite{30440} \\
4.10 & 4440& \emph{ i }& 23.39 $\pm$ 0.14 & DOLORES/TNG & \cite{30432} \\
4.10 & 4440& \emph{ r }& 23.35 $\pm$ 0.16 & DOLORES/TNG & \cite{30432} \\
4.45 & 840& \emph{ K }& 23.00 $\pm$ 0.30 & NIRI/Gemini-North & This work \\
5.10 & 1020& \emph{ r }& 23.68 $\pm$ 0.10 & OSIRIS/GTC & This work \\%(Alan 2022-03-13) \\
5.11 & 1020& \emph{ z }& 22.56 $\pm$ 0.15 & OSIRIS/GTC & This work \\%(Nat 2022-03-17) \\
5.50 & 1440& \emph{ J }& 22.20 $\pm$ 0.30 & NIRI/Gemini-North & This work \\
6.08 & 900& \emph{ g }& 23.78 $\pm$ 0.11 & AlFOSC/NOT & \cite{30443} \\
6.10 & 900& \emph{ r }& 23.27 $\pm$ 0.09 & AlFOSC/NOT & \cite{30443} \\
6.35 & 1500& \emph{ r }& 23.14 $\pm$ 0.27 & LMI/LDT & This work \\%(Alan 2021-08-19)\\
6.45 & 2580& \emph{ K }& 23.10 $\pm$ 0.20  & NIRI/Gemini-North & This work \\
6.98 & 3600& \emph{ R }& 23.10 $\pm$ 0.30 & Zeiss-1000/SAO-RAS & \cite{30465} \\
10.44 & 1080& \emph{ r }& 23.73 $\pm$ 0.10 & GMOS-N/Gemini-North & This work \\%(Alan 2022-03-13)\\
11.44 & 900& \emph{ z }& $>$ 22.44 & GMOS-N/Gemini-North & This work \\%(Nat)\\
12.45 & 1800 & \emph{ K }& 23.10 $\pm$ 0.20 & NIRI/Gemini-North & This work \\
14.45 & 1584& \emph{ z }& 23.58 $\pm$ 0.24 & GMOS-N/Gemini-North & This work \\%(Nat 2022-03-13)\\
115.00 & 3030& \emph{ r }& $>$ 25.21 & HSC/Subaru & This work \\
161 & 7200 &\emph{ K } & $>24.0$ & NIRI/Gemini-North & This work \\



==> GRB 210704A/references.tex <==
\bibitem[\protect\citeauthoryear{Abbott et al.}{2017a}]{Abbott2017} Abbott B.~P., et al., 2017a, PhRvL, 119, 161101

%\bibitem[\protect\citeauthoryear{Ahumada et al.}{2021}]{Ahumada2021} Ahumada T., Singer L.~P., Anand S., Coughlin M.~W., Kasliwal M.~M., Ryan G., Andreoni I., et al., 2021, arXiv, arXiv:2105.05067
\bibitem[\protect\citeauthoryear{Adams et al.}{2017}]{Adams2017} Adams S.~M., Kochanek C.~S., Gerke J.~R., Stanek K.~Z., 2017, MNRAS, 469, 1445. doi:10.1093/mnras/stx898

\bibitem[\protect\citeauthoryear{Ahumada et al.}{2020}]{SDSS16} Ahumada R., Prieto C.~A., Almeida A., Anders F., Anderson S.~F., Andrews B.~H., Anguiano B., et al., 2020, ApJS, 249, 3. doi:10.3847/1538-4365/ab929e

\bibitem[Ahumada et al.(2021)]{Ahumada2021} Ahumada, T., Singer, L.~P., Anand, S., et al.\ 2021, Nature Astronomy, 5, 917. doi:10.1038/s41550-021-01428-7


\bibitem[\protect\citeauthoryear{Alam et al.}{2015}]{SDSS12} Alam S., Albareti F.~D., Allende Prieto C., Anders F., Anderson S.~F., Anderton T., Andrews B.~H., et al., 2015, ApJS, 219, 12. doi:10.1088/0067-0049/219/1/12

\bibitem[\protect\citeauthoryear{Amati et al.}{2008}]{Amati2008} Amati L., Guidorzi C., Frontera F., Della Valle M., Finelli F., Landi R., Montanari E., 2008, MNRAS, 391, 577. doi:10.1111/j.1365-2966.2008.13943.x

\bibitem[Antonelli et al.(2009)]{Antonelli09} Antonelli, L.~A., D'Avanzo, P., Perna, R., et al.\ 2009, \aap, 507, L45. doi:10.1051/0004-6361/200913062

\bibitem[\protect\citeauthoryear{Arnett}{1982}]{Arnett1982} Arnett W.~D., 1982, ApJ, 253, 785. doi:10.1086/159681

\bibitem[\protect\citeauthoryear{Barbieri et al.}{2019}]{Barbieri2019} Barbieri C., Salafia O.~S., Colpi M., Ghirlanda G., Perego A., Colombo A., 2019, ApJL, 887, L35. doi:10.3847/2041-8213/ab5c1e

\bibitem[\protect\citeauthoryear{Becerra et al.}{2017}]{Becerra2017} Becerra R.~L., Watson A.~M., Lee W.~H., Fraija N., Butler N.~R., Bloom J.~S., Capone J.~I., et al., 2017, ApJ, 837, 116. doi:10.3847/1538-4357/aa610f

\bibitem[\protect\citeauthoryear{Beckwith et al.}{2006}]{Beckwith2006} Beckwith S.~V.~W., Stiavelli M., Koekemoer A.~M., Caldwell J.~A.~R., Ferguson H.~C., Hook R., Lucas R.~A., et al., 2006, AJ, 132, 1729. doi:10.1086/507302

\bibitem[\protect\citeauthoryear{Beniamini et al.}{2015}]{Beniamini2015} Beniamini P., Nava L., Duran R.~B., Piran T., 2015, MNRAS, 454, 1073. doi:10.1093/mnras/stv2033

\bibitem[\protect\citeauthoryear{Berger}{2010}]{Berger2010} Berger E., 2010, ApJ, 722, 1946. doi:10.1088/0004-637X/722/2/1946

\bibitem[\protect\citeauthoryear{Berger et al.}{2011}]{Berger2011} Berger E., Chornock R., Holmes T.~R., Foley R.~J., Cucchiara A., Wolf C., Podsiadlowski P., et al., 2011, ApJ, 743, 204. doi:10.1088/0004-637X/743/2/204

\bibitem[\protect\citeauthoryear{Berretta et al.}{2021}]{30375} Berretta A., Longo F., Axelsson M., Bissaldi E., Piron F., Arimoto M., Fermi-LAT Collaboration, 2021, GCN, 30375

\bibitem[\protect\citeauthoryear{Bertin \& Arnouts}{1996}]{Bertin1996} Bertin E., Arnouts S., 1996, A\&AS, 117, 393

\bibitem[\protect\citeauthoryear{Bloom, Kulkarni, \& Djorgovski}{2002}]{Bloom2002} Bloom J.~S., Kulkarni S.~R., Djorgovski S.~G., 2002, AJ, 123, 1111. doi:10.1086/338893

\bibitem[\protect\citeauthoryear{Bloom et al.}{2006}]{Bloom2006} Bloom J.~S., Prochaska J.~X., Pooley D., Blake C.~H., Foley R.~J., Jha S., Ramirez-Ruiz E., et al., 2006, ApJ, 638, 354. doi:10.1086/498107


%\bibitem[\protect\citeauthoryear{Bradley et al.}{2001}]{Bradley2021} Bradley, L., 2021, astropy/photutils: 1.1.0. doi:10.5281/zenodo.4624996

\bibitem[\protect\citeauthoryear{Breeveld, Lien, \& Swift/UVOT Team}{2021}]{30389} Breeveld A.~A., Lien A.~Y., Swift/UVOT Team, 2021, GCN, 30389

\bibitem[\protect\citeauthoryear{Burenin et al.}{2007}]{ROSAT} Burenin R.~A., Vikhlinin A., Hornstrup A., Ebeling H., Quintana H., Mescheryakov A., 2007, ApJS, 172, 561. doi:10.1086/519457

\bibitem[\protect\citeauthoryear{Campana et al.}{2006}]{Campana2006} Campana S., Mangano V., Blustin A.~J., Brown P., Burrows D.~N., Chincarini G., Cummings J.~R., et al., 2006, Natur, 442, 1008. doi:10.1038/nature04892

\bibitem[\protect\citeauthoryear{Cartier et al.}{2021}]{Cartier2021} Cartier R., Hamuy M., Contreras C., Anderson J.~P., Phillips M.~M., Morrell N., Stritzinger M.~D., et al., 2021, arXiv, arXiv:2108.09828

\bibitem[\protect\citeauthoryear{Cucchiara et al.}{2013}]{Cucchiara2013} Cucchiara A., Prochaska J.~X., Zhu G., M{\'e}nard B., Fynbo J.~P.~U., Fox D.~B., Chen H.-W., et al., 2013, ApJ, 773, 82. doi:10.1088/0004-637X/773/2/82

\bibitem[\protect\citeauthoryear{Cutri et al.}{2003}]{Cutri2003} Cutri R.~M., Skrutskie M.~F., van Dyk S., Beichman C.~A., Carpenter J.~M., Chester T., Cambresy L., et al., 2003, tmc..book

\bibitem[\protect\citeauthoryear{D'Ai et al.}{2021}]{30379} D'Ai A., Kennea J.~A., Tohuvavohu A., Sbarufatti B., Page K.~L., Beardmore A.~P., Melandri A., et al., 2021, GCN, 30379

\bibitem[\protect\citeauthoryear{D'Avanzo et al.}{2021}]{30385} D'Avanzo P., D'Elia V., Fiorenzano A., Padilla C., CIBO Collaboration, 2021, GCN, 30385

\bibitem[\protect\citeauthoryear{D'Avanzo et al.}{2021}]{30432} D'Avanzo P., D'Elia V., Campana S., De Pasquale M., Melandri A., Rossi A., Salvaterra R., et al., 2021, GCN, 30432

\bibitem[\protect\citeauthoryear{de Ugarte Postigo et al.}{2012}]{deUgarte2012} de Ugarte Postigo A., Fynbo J.~P.~U., Th{\"o}ne C.~C., Christensen L., Gorosabel J., Milvang-Jensen B., Schulze S., et al., 2012, A\&A, 548, A11. doi:10.1051/0004-6361/201219894

\bibitem[\protect\citeauthoryear{de Ugarte Postigo et al.}{2014}]{deUgarte2014} de Ugarte Postigo A., Blazek M., Janout P., Sprimont P., Th{\"o}ne C.~C., Gorosabel J., S{\'a}nchez-Ram{\'\i}rez R., 2014, SPIE, 9152, 91520B. doi:10.1117/12.2055774

\bibitem[\protect\citeauthoryear{de Ugarte Postigo et al.}{2021}]{30392} de Ugarte Postigo A., Kann D.~A., Thoene C., Blazek M., Agui Fernandez J.~F., Fynbo J.~P.~U., Izzo L., et al., 2021, GCN, 30392

\bibitem[\protect\citeauthoryear{Dichiara et al.}{2021}]{30383} Dichiara S., Troja E., Butler N., Watson A.~M., Becerra R.~L., Kutyrev A., Lee W.~H., et al., 2021, GCN, 30383

\bibitem[\protect\citeauthoryear{Dichiara et al.}{2021}]{Dichiara2021} Dichiara S., Troja E., Lipunov V., Ricci R., Oates S.~R., Butler N.~R., Liuzzo E., et al., 2021, arXiv, arXiv:2111.14861

\bibitem[\protect\citeauthoryear{Dimple et al.}{2022}]{Dimple2022} Dimple, Misra K., Ghosh A., Arun K.~G., Gupta R., Kumar A., Resmi L., et al., 2022, arXiv, arXiv:2202.01191. doi:10.48550/arXiv.2202.01191

\bibitem[\protect\citeauthoryear{Drout et al.}{2017}]{Drout17} Drout M.~R., Piro A.~L., Shappee B.~J., Kilpatrick C.~D., Simon J.~D., Contreras C., Coulter D.~A., et al., 2017, Sci, 358, 1570. doi:10.1126/science.aaq0049

\bibitem[\protect\citeauthoryear{Eichler et al.}{1989}]{Eichler1989} Eichler D., Livio M., Piran T., Schramm D.~N., 1989, Natur, 340, 126. doi:10.1038/340126a0

\bibitem[\protect\citeauthoryear{Evans et al.}{2009}]{Evans2009} Evans P.~A., Beardmore A.~P., Page K.~L., Osborne J.~P., O'Brien P.~T., Willingale R., Starling R.~L.~C., et al., 2009, MNRAS, 397, 1177. doi:10.1111/j.1365-2966.2009.14913.x

\bibitem[\protect\citeauthoryear{Evans et al.}{2017}]{Evans17} Evans P.~A., Cenko S.~B., Kennea J.~A., Emery S.~W.~K., Kuin N.~P.~M., Korobkin O., Wollaeger R.~T., et al., 2017, Sci, 358, 1565. doi:10.1126/science.aap9580

\bibitem[\protect\citeauthoryear{Evans \& Swift Team}{2021}]{30374} Evans P.~A., Swift Team, 2021, GCN, 30374

\bibitem[\protect\citeauthoryear{Fong, Berger, \& Fox}{2010}]{Fong2010} Fong W., Berger E., Fox D.~B., 2010, ApJ, 708, 9. doi:10.1088/0004-637X/708/1/9

\bibitem[\protect\citeauthoryear{Fong \& Rastinejad}{2021}]{30445} Fong W., Rastinejad J., 2021, GCN, 30445

\bibitem[\protect\citeauthoryear{Fraija}{2015}]{Fraija2015} Fraija N., 2015, ApJ, 804, 105. doi:10.1088/0004-637X/804/2/105

\bibitem[\protect\citeauthoryear{Fryer, Burrows, \& Benz}{1998}]{Fryer1998} Fryer C., Burrows A., Benz W., 1998, ApJ, 496, 333. doi:10.1086/305348

\bibitem[\protect\citeauthoryear{Fryer, Hungerford, \& Young}{2007}]{Fryer2007} Fryer C.~L., Hungerford A.~L., Young P.~A., 2007, ApJL, 662, L55. doi:10.1086/519523


\bibitem[\protect\citeauthoryear{Fynbo et al.}{2009}]{Fynbo2009} Fynbo J.~P.~U., Jakobsson P., Prochaska J.~X., Malesani D., Ledoux C., de Ugarte Postigo A., Nardini M., et al., 2009, ApJS, 185, 526. doi:10.1088/0067-0049/185/2/526


\bibitem[\protect\citeauthoryear{Galama et al.}{1998}]{Galama1998} Galama T.~J., Vreeswijk P.~M., van Paradijs J., Kouveliotou C., Augusteijn T., B{\"o}hnhardt H., Brewer J.~P., et al., 1998, Nature, 395, 670. doi:10.1038/27150

\bibitem[\protect\citeauthoryear{Garcia-Cifuentes et al.}{2023}]{Garcia-Cifuentes2023} Garcia-Cifuentes K., Becerra R.~L., De Colle F., Cabrera J. I., del Burgo C., 2023, arXiv, arXiv:2304.08666

\bibitem[\protect\citeauthoryear{Gehrels et al.}{2005}]{Gehrels2005} Gehrels N., Sarazin C.~L., O'Brien P.~T., Zhang B., Barbier L., Barthelmy S.~D., Blustin A., et al., 2005, Natur, 437, 851. doi:10.1038/nature04142

\bibitem[\protect\citeauthoryear{Gehrels et al.}{2006}]{Gehrels2006} Gehrels N., Norris J.~P., Barthelmy S.~D., Granot J., Kaneko Y., Kouveliotou C., Markwardt C.~B., et al., 2006, Natur, 444, 1044. doi:10.1038/nature05376

\bibitem[\protect\citeauthoryear{Gehrels \& Razzaque}{2013}]{Gehrels2013} Gehrels N., Razzaque S., 2013, FrPhy, 8, 661. doi:10.1007/s11467-013-0282-3

\bibitem[\protect\citeauthoryear{Giacomazzo, Rezzolla, \& Stergioulas}{2011}]{Giacomazzo2011} Giacomazzo B., Rezzolla L., Stergioulas N., 2011, PhRvD, 84, 024022. doi:10.1103/PhysRevD.84.024022

\bibitem[\protect\citeauthoryear{Gonzaga et al.}{2012}]{Gonzaga2012} Gonzaga S., Hack W., Fruchter A., Mack J., 2012, drzp.book

\bibitem[\protect\citeauthoryear{Granot \& Sari}{2002}]{Granot2002} Granot J., Sari R., 2002, ApJ, 568, 820. doi:10.1086/338966

\bibitem[\protect\citeauthoryear{Grossman et al.}{2014}]{Grossman2014} Grossman D., Korobkin O., Rosswog S., Piran T., 2014, MNRAS, 439, 757. doi:10.1093/mnras/stt2503

\bibitem[\protect\citeauthoryear{Hakkila et al.}{2018}]{Hakkila+18smoke} Hakkila J., Lesage S., McAfee S., Hofesmann E., Maly Taylor C., Cannon T., 2018, ApJ, 863, 77. doi:10.3847/1538-4357/aad335

\bibitem[\protect\citeauthoryear{Hjorth \& Bloom}{2012}]{Hjorth2012} Hjorth J., Bloom J.~S., 2012, grb..book, 169

\bibitem[Ho et al.(2020)]{Ho2020} Ho, A.~Y.~Q., Perley, D.~A., Kulkarni, S.~R., et al.\ 2020, \apj, 895, 49. doi:10.3847/1538-4357/ab8bcf

\bibitem[\protect\citeauthoryear{Hosseinzadeh et al.}{2017}]{Hosseinzadeh2017} Hosseinzadeh G., Arcavi I., Valenti S., McCully C., Howell D.~A., Johansson J., Sollerman J., et al., 2017, ApJ, 836, 158. doi:10.3847/1538-4357/836/2/158


\bibitem[\protect\citeauthoryear{Johnson et al.}{2019}]{Johnson2019} Johnson B.~D., Leja J.~L., Conroy C., Speagle J.~S., 2019, ascl.soft

\bibitem[\protect\citeauthoryear{Kashikawa et al.}{2004}]{Kashikawa2004} Kashikawa N., Shimasaku K., Yasuda N., Ajiki M., Akiyama M., Ando H., Aoki K., et al., 2004, PASJ, 56, 1011. doi:10.1093/pasj/56.6.1011

\bibitem[\protect\citeauthoryear{Kann et al.}{2021}]{30391} Kann D.~A., de Ugarte Postigo A., Thoene C., Blazek M., Agui Fernandez J.~F., Martin-Fernandez P., 2021, GCN, 30391

\bibitem[\protect\citeauthoryear{Kann et al.}{2021}]{30401} Kann D.~A., de Ugarte Postigo A., Thoene C., Blazek M., Agui Fernandez J.~F., Maicas N., Lamadrid (COAJ J.~L., 2021, GCN, 30401

\bibitem[\protect\citeauthoryear{Kann et al.}{2021}]{30443} Kann D.~A., Izzo L., Galindo Guil F.~J., Kasikov A., 2021, GCN, 30443

\bibitem[\protect\citeauthoryear{Kim et al.}{2021}]{30384} Kim V., Pozanenko A., Krugov M., Belkin S., Pankov N., IKI FuN G., 2021, GCN, 30384

\bibitem[\protect\citeauthoryear{King, Olsson, \& Davies}{2007}]{King2007} King A., Olsson E., Davies M.~B., 2007, MNRAS, 374, L34. doi:10.1111/j.1745-3933.2006.00259.x

\bibitem[\protect\citeauthoryear{Kouveliotou, et al.}{1993}]{Kouveliotou93} Kouveliotou C., et al., 1993, ApJL, 413, L101

\bibitem[\protect\citeauthoryear{Kumar \& Piran}{2000}]{Kumar2000} Kumar P., Piran T., 2000, ApJ, 532, 286. doi:10.1086/308537

\bibitem[\protect\citeauthoryear{Kunzweiler et al.}{2021}]{30369} Kunzweiler F., Biltzinger B., Berlato F., Burgess J., Greiner J., 2021, GCN, 30369

\bibitem[\protect\citeauthoryear{Le F{\`e}vre et al.}{2004}]{LeFevre2004} Le F{\`e}vre O., Vettolani G., Paltani S., Tresse L., Zamorani G., Le Brun V., Moreau C., et al., 2004, A\&A, 428, 1043. doi:10.1051/0004-6361:20048072


\bibitem[\protect\citeauthoryear{Lee \& Ramirez-Ruiz}{2007}]{Lee2007} Lee W.~H., Ramirez-Ruiz E., 2007, NJPh, 9, 17. doi:10.1088/1367-2630/9/1/017

\bibitem[\protect\citeauthoryear{Levan et al.}{2006}]{Levan2006} Levan A.~J., Wynn G.~A., Chapman R., Davies M.~B., King A.~R., Priddey R.~S., Tanvir N.~R., 2006, MNRAS, 368, L1. doi:10.1111/j.1745-3933.2006.00144.x

\bibitem[\protect\citeauthoryear{Levan et al.}{2021}]{30381} Levan A.~J., Campana S., Kann D.~A., D'Avanzo P., 2021, GCN, 30381

\bibitem[\protect\citeauthoryear{Levesque}{2014}]{Levesque2014} Levesque E.~M., 2014, PASP, 126, 1. doi:10.1086/674531

\bibitem[\protect\citeauthoryear{Lyutikov \& Toonen}{2019}]{LyutikovToonen2019} Lyutikov M., Toonen S., 2019, MNRAS, 487, 5618. doi:10.1093/mnras/stz1640

\bibitem[\protect\citeauthoryear{MacFadyen \& Woosley}{1999}]{MacFadyen1999ApJ} MacFadyen A.~I., Woosley S.~E., 1999, ApJ, 524, 262. doi:10.1086/307790

\bibitem[\protect\citeauthoryear{Malacaria, Meegan, \& Fermi GBM Team}{2021}]{30380} Malacaria C., Meegan C., Fermi GBM Team, 2021, GCN, 30380

\bibitem[\protect\citeauthoryear{Mazzali et al.}{2006}]{Mazzali2006} Mazzali P.~A., Deng J., Nomoto K., Sauer D.~N., Pian E., Tominaga N., Tanaka M., et al., 2006, Natur, 442, 1018. doi:10.1038/nature05081

\bibitem[\protect\citeauthoryear{McCracken et al.}{2003}]{McCracken2003} McCracken H.~J., Radovich M., Bertin E., Mellier Y., Dantel-Fort M., Le F{\`e}vre O., Cuillandre J.~C., et al., 2003, A\&A, 410, 17. doi:10.1051/0004-6361:20031081

\bibitem[\protect\citeauthoryear{Mendel et al.}{2014}]{Mendel2014} Mendel J.~T., Simard L., Palmer M., Ellison S.~L., Patton D.~R., 2014, ApJS, 210, 3

\bibitem[\protect\citeauthoryear{Metcalfe et al.}{2001}]{Metcalfe2001} Metcalfe N., Shanks T., Campos A., McCracken H.~J., Fong R., 2001, MNRAS, 323, 795. doi:10.1046/j.1365-8711.2001.04168.x

\bibitem[\protect\citeauthoryear{Minaev \& Pozanenko}{2020}]{Minaev2020} Minaev P.~Y., Pozanenko A.~S., 2020, MNRAS, 492, 1919. doi:10.1093/mnras/stz3611

\bibitem[\protect\citeauthoryear{Minaev et al.}{2021a}]{30444} Minaev, Pozanenko, Chelovekov, Grebenev, GRB IKI FuN, 2021, GCN, 30444

\bibitem[\protect\citeauthoryear{Minaev et al.}{2021b}]{30452} Minaev P., Pozanenko A., Chelovekov I., Grebenev S., GRB IKI FuN, 2021, GCN, 30452

\bibitem[\protect\citeauthoryear{Mirabal et al.}{2006}]{Mirabal2006} Mirabal N., Halpern J.~P., An D., Thorstensen J.~R., Terndrup D.~M., 2006, ApJL, 643, L99. doi:10.1086/505177

\bibitem[\protect\citeauthoryear{Miyazaki et al.}{2018}]{Miyazaki2018} Miyazaki S., Komiyama Y., Kawanomoto S., Doi Y., Furusawa H., Hamana T., Hayashi Y., et al., 2018, PASJ, 70, S1. doi:10.1093/pasj/psx063

\bibitem[\protect\citeauthoryear{Moss et al.}{2022}]{Moss2022} Moss M., Lien A., Guiriec S., Cenko S.~B., Sakamoto T., 2022, ApJ, 927, 157. doi:10.3847/1538-4357/ac4d94

\bibitem[Nakar \& Piran(2017)]{nakar17} Nakar, E. \& Piran, T.\ 2017, \apj, 834, 28. doi:10.3847/1538-4357/834/1/28

\bibitem[\protect\citeauthoryear{Narayan, Paczynski, \& Piran}{1992}]{Narayan1992} Narayan R., Paczynski B., Piran T., 1992, ApJL, 395, L83. doi:10.1086/186493

\bibitem[\protect\citeauthoryear{Norris, Marani, \& Bonnell}{2000}]{Norris2000} Norris J.~P., Marani G.~F., Bonnell J.~T., 2000, ApJ, 534, 248. doi:10.1086/308725

\bibitem[\protect\citeauthoryear{Norris}{2002}]{Norris2002} Norris J.~P., 2002, ApJ, 579, 386. doi:10.1086/342747

\bibitem[\protect\citeauthoryear{O'Connor, Beniamini, \& Kouveliotou}{2020}]{OConnor2020} O'Connor B., Beniamini P., Kouveliotou C., 2020, MNRAS, 495, 4782. doi:10.1093/mnras/staa1433

\bibitem[\protect\citeauthoryear{O'Connor et al.}{2021}]{OConnor2021} O'Connor B., Troja E., Dichiara S., Chase E.~A., Ryan G., Cenko S.~B., Fryer C.~L., et al., 2021, MNRAS, 502, 1279. doi:10.1093/mnras/stab132

\bibitem[\protect\citeauthoryear{O'Connor et al.}{2021}]{30451}
O'Connor, B., Troja, E., Zack, E., Dichiara, S., Gatkine, P., Durbak J.~M., Cenko, S.~B., Kutyrev, A., \& Veilleux, S. 2021, GCN, 30451

\bibitem[\protect\citeauthoryear{O'Connor et al.}{2022}]{OConnor2022} O'Connor B., Troja E., Dichiara S., Beniamini P., Cenko S.~B., Kouveliotou C., Gonz{\'a}lez J.~B., et al., 2022, MNRAS.tmp. doi:10.1093/mnras/stac1982

\bibitem[\protect\citeauthoryear{O'Connor et al.}{2023}]{OConnor2023} O'Connor B., Troja E., Ryan G., Beniamini P., van Eerten H., Granot J., Dichiara S., et al., 2023, arXiv, arXiv:2302.07906. doi:10.48550/arXiv.2302.07906

\bibitem[\protect\citeauthoryear{Page et al.}{2006}]{Page2006} Page K.~L., King A.~R., Levan A.~J., O'Brien P.~T., Osborne J.~P., Barthelmy S.~D., Beardmore A.~P., et al., 2006, ApJL, 637, L13. doi:10.1086/500430

\bibitem[\protect\citeauthoryear{Palmerio, et al.}{2019}]{Palmerio2019} Palmerio J.~T., et al., 2019, A\&A, 623, A26

\bibitem[\protect\citeauthoryear{Pankov et al.}{2021}]{30440} Pankov N., Belkin S., Kim V., Pozanenko A., Krugov M., GRB IKI FuN, 2021, GCN, 30440

\bibitem[\protect\citeauthoryear{Pastorello et al.}{2010}]{Pastorello2010} Pastorello A., Smartt S.~J., Botticella M.~T., Maguire K., Fraser M., Smith K., Kotak R., et al., 2010, ApJL, 724, L16. doi:10.1088/2041-8205/724/1/L16


\bibitem[\protect\citeauthoryear{Perley et al.}{2019}]{Perley2019} Perley D.~A., Mazzali P.~A., Yan L., Cenko S.~B., Gezari S., Taggart K., Blagorodnova N., et al., 2019, MNRAS, 484, 1031. doi:10.1093/mnras/sty3420

\bibitem[\protect\citeauthoryear{Perley et al.}{2021}]{Perley2021} Perley D.~A., Ho A.~Y.~Q., Yao Y., Fremling C., Anderson J.~P., Schulze S., Kumar H., et al., 2021, MNRAS, 508, 5138. doi:10.1093/mnras/stab2785

\bibitem[\protect\citeauthoryear{Planck Collaboration et al.}{2014}]{Planck2014} Planck Collaboration, Ade P.~A.~R., Aghanim N., Alves M.~I.~R., Armitage-Caplan C., Arnaud M., Ashdown M., et al., 2014, A\&A, 571, A1. doi:10.1051/0004-6361/201321529

\bibitem[\protect\citeauthoryear{Poolakkil et al.}{2021}]{Poolakkil2021} Poolakkil S., Preece R., Fletcher C., Goldstein A., Bhat P.~N., Bissaldi E., Briggs M.~S., et al., 2021, ApJ, 913, 60. doi:10.3847/1538-4357/abf24d

\bibitem[\protect\citeauthoryear{Prasad et al.}{2021}]{30378} Prasad V., Sawant P., Waratkar G., Vibhute A., Bhalerao V., Bhattacharya D., Rao A.~R., et al., 2021, GCN, 30378

\bibitem[\protect\citeauthoryear{Qin et al.}{2013}]{Qin2013} Qin Y., Liang E.-W., Liang Y.-F., Yi S.-X., Lin L., Zhang B.-B., Zhang J., et al., 2013, ApJ, 763, 15. doi:10.1088/0004-637X/763/1/15

\bibitem[\protect\citeauthoryear{Rastinejad et al.}{2021}]{Rastinejad2021} Rastinejad J.~C., Fong W., Kilpatrick C.~D., Paterson K., Tanvir N.~R., Levan A.~J., Metzger B.~D., et al., 2021, ApJ, 916, 89. doi:10.3847/1538-4357/ac04b4

\bibitem[\protect\citeauthoryear{Rastinejad et al.}{2021}]{30433} Rastinejad J., Levan A., Fong W., Tanvir N.~R., Rouco Escorial A., 2021, GCN, 30433

\bibitem[\protect\citeauthoryear{Richardson et al.}{2014}]{Richardson2014} Richardson D., Jenkins R.~L., Wright J., Maddox L., 2014, AJ, 147, 118. doi:10.1088/0004-6256/147/5/118

\bibitem[\protect\citeauthoryear{Richmond et al.}{1996}]{Richmon1996} Richmond M.~W., van Dyk S.~D., Ho W., Peng C.~Y., Paik Y., Treffers R.~R., Filippenko A.~V., et al., 1996, AJ, 111, 327. doi:10.1086/117785

\bibitem[\protect\citeauthoryear{Ridnaia et al.}{2021}]{30388} Ridnaia A., Frederiks D., Golenetskii S., Lysenko A., Svinkin D., Tsvetkova A., Ulanov M., et al., 2021, GCN, 30388

\bibitem[\protect\citeauthoryear{Rosswog \& Ramirez-Ruiz}{2002}]{Rosswog2002} Rosswog S., Ramirez-Ruiz E., 2002, MNRAS, 336, L7. doi:10.1046/j.1365-8711.2002.05898.x

\bibitem[\protect\citeauthoryear{Rueda et al.}{2018}]{Rueda2018} Rueda J.~A., Ruffini R., Wang Y., Aimuratov Y., Barres de Almeida U., Bianco C.~L., Chen Y.~C., et al., 2018, JCAP, 2018, 006. doi:10.1088/1475-7516/2018/10/006

\bibitem[\protect\citeauthoryear{Ruffert \& Janka}{1998}]{Ruffert1998} Ruffert M., Janka H.-T., 1998, A\&A, 338, 535

\bibitem[\protect\citeauthoryear{Salafia et al.}{2021}]{Salafia2021} Salafia O.~S., Ravasio M.~E., Yang J., An T., Orienti M., Ghirlanda G., Nava L., et al., 2021, arXiv, arXiv:2106.07169

\bibitem[\protect\citeauthoryear{Sari, Piran, \& Narayan}{1998}]{Sari1998} Sari R., Piran T., Narayan R., 1998, ApJL, 497, L17. doi:10.1086/311269

\bibitem[\protect\citeauthoryear{Savaglio, Glazebrook, \& Le Borgne}{2009}]{Savaglio09} Savaglio S., Glazebrook K., Le Borgne D., 2009, ApJ, 691, 182. doi:10.1088/0004-637X/691/1/182

\bibitem[\protect\citeauthoryear{Schlegel, Finkbeiner, \& Davis}{1998}]{Schlegel1998} Schlegel D.~J., Finkbeiner D.~P., Davis M., 1998, ApJ, 500, 525. doi:10.1086/305772

\bibitem[\protect\citeauthoryear{Sharon \& Kushnir}{2020}]{SharonKushnir2020} Sharon A., Kushnir D., 2020, ApJ, 894, 146. doi:10.3847/1538-4357/ab8a31

\bibitem[\protect\citeauthoryear{Speagle}{2020}]{dynesty} Speagle J.~S., 2020, MNRAS, 493, 3132.

\bibitem[\protect\citeauthoryear{Sun et al.}{2021}]{30411} Sun T.-R., Hu Y.-D., Fernandez-Garcia E., Caballero-Garcia A.~J.~C.-T.~M.~D., Castro Tirado M.~A., Martin-Fernandez P., 2021, GCN, 30411

\bibitem[\protect\citeauthoryear{Tanvir et al.}{2013}]{Tanvir13} Tanvir N.~R., Levan A.~J., Fruchter A.~S., Hjorth J., Hounsell R.~A., Wiersema K., Tunnicliffe R.~L., 2013, Natur, 500, 547. doi:10.1038/nature12505

\bibitem[\protect\citeauthoryear{Toba et al.}{2014}]{Toba2014} Toba Y., Oyabu S., Matsuhara H., Malkan M.~A., Gandhi P., Nakagawa T., Isobe N., et al., 2014, ApJ, 788, 45. doi:10.1088/0004-637X/788/1/45

\bibitem[\protect\citeauthoryear{Troja et al.}{2008}]{Troja2008} Troja E., King A.~R., O'Brien P.~T., Lyons N., Cusumano G., 2008, MNRAS, 385, L10. doi:10.1111/j.1745-3933.2007.00421.x

\bibitem[\protect\citeauthoryear{Troja et al.}{2012}]{Troja2012} Troja E., Sakamoto T., Guidorzi C., Norris J.~P., Panaitescu A., Kobayashi S., Omodei N., et al., 2012, ApJ, 761, 50. doi:10.1088/0004-637X/761/1/50

\bibitem[\protect\citeauthoryear{Troja et al.}{2019}]{Troja2019} Troja E., Castro-Tirado A.~J., Becerra Gonz{\'a}lez J., Hu Y., Ryan G.~S., Cenko S.~B., Ricci R., et al., 2019, MNRAS, 489, 2104. doi:10.1093/mnras/stz2255

\bibitem[\protect\citeauthoryear{Troja et al.}{2021}]{30390} Troja E., Butler N., Watson A.~M., Kutyrev A., Lee W.~H., Richer M.~G., Fox O., et al., 2021, GCN, 30390

\bibitem[\protect\citeauthoryear{Troja et al.}{2022}]{Troja2022} Troja E., Fryer C.~L., O'Connor B., Ryan G., Dichiara S., Kumar A., Ito N., et al., 2022, Natur, 612, 228. doi:10.1038/s41586-022-05327-3

\bibitem[\protect\citeauthoryear{Troja, Watson, \& O'Connor}{2021}]{30442} Troja E., Watson A., O'Connor B., 2021, GCN, 30442

\bibitem[\protect\citeauthoryear{Tundo et al.}{2012}]{Tundo2012} Tundo E., Moretti A., Tozzi P., Teng L., Rosati P., Tagliaferri G., Campana S., 2012, A\&A, 547, A57. doi:10.1051/0004-6361/201219038

\bibitem[\protect\citeauthoryear{Tunnicliffe et al.}{2014}]{Tunnicliffe2014} Tunnicliffe R.~L., Levan A.~J., Tanvir N.~R., Rowlinson A., Perley D.~A., Bloom J.~S., Cenko S.~B., et al., 2014, MNRAS, 437, 1495. doi:10.1093/mnras/stt1975


\bibitem[\protect\citeauthoryear{Ukwatta et al.}{2010}]{Ukwatta+10lag} Ukwatta T.~N., Stamatikos M., Dhuga K.~S., Sakamoto T., Barthelmy S.~D., Eskandarian A., Gehrels N., et al., 2010, ApJ, 711, 1073. doi:10.1088/0004-637X/711/2/1073


\bibitem[\protect\citeauthoryear{Ursi et al.}{2021}]{30372} Ursi A., Pittori C., Verrecchia F., Tavani M., Argan A., Cardillo M., Casentini C., et al., 2021, GCN, 30372

\bibitem[\protect\citeauthoryear{Valenti et al.}{2008}]{Valenti2008} Valenti S., Benetti S., Cappellaro E., Patat F., Mazzali P., Turatto M., Hurley K., et al., 2008, MNRAS, 383, 1485. doi:10.1111/j.1365-2966.2007.12647.x


\bibitem[\protect\citeauthoryear{Villar et al.}{2017}]{Villar2017} Villar V.~A., Guillochon J., Berger E., Metzger B.~D., Cowperthwaite P.~S., Nicholl M., Alexander K.~D., et al., 2017, ApJL, 851, L21. doi:10.3847/2041-8213/aa9c84

\bibitem[\protect\citeauthoryear{Vink{\'o} et al.}{2015}]{Vinko2015} Vink{\'o} J., Yuan F., Quimby R.~M., Wheeler J.~C., Ramirez-Ruiz E., Guillochon J., Chatzopoulos E., et al., 2015, ApJ, 798, 12. doi:10.1088/0004-637X/798/1/12

\bibitem[\protect\citeauthoryear{Volnova et al.}{2021}]{30465} Volnova A., Moskvitin A., Pozanenko A., Pankov N., Belkin S., IKI FuN G., 2021, GCN, 30465

\bibitem[\protect\citeauthoryear{Watson et al.}{2021}]{30436} Watson A.~M., Troja E., Becerra R.~L., S{\'a}nchez R., Thakur A., Dichiara S., Butler N., et al., 2021, GCN, 30436

\bibitem[\protect\citeauthoryear{Williams et al.}{2023}]{Williams2023} Williams M.~A., Kennea J.~A., Dichiara S., Kobayashi K., Iwakiri W.~B., Beardmore A.~P., Evans P.~A., et al., 2023, arXiv, arXiv:2302.03642. doi:10.48550/arXiv.2302.03642

\bibitem[\protect\citeauthoryear{Wollaeger et al.}{2021}]{Wollaeger2021} Wollaeger R.~T., Fryer C.~L., Chase E.~A., Fontes C.~J., Ristic M., Hungerford A.~L., Korobkin O., et al., 2021, ApJ, 918, 10. doi:10.3847/1538-4357/ac0d03

\bibitem[\protect\citeauthoryear{Woosley}{1993}]{Woosley1993} Woosley S.~E., 1993, ApJ, 405, 273. doi:10.1086/172359

\bibitem[\protect\citeauthoryear{Woosley \& Bloom}{2006}]{Woosley2006} Woosley S.~E., Bloom J.~S., 2006, ARA\&A, 44, 507. doi:10.1146/annurev.astro.43.072103.150558

\bibitem[\protect\citeauthoryear{Yang et al.}{2022}]{Yang2022} Yang J., Ai S., Zhang B.-B., Zhang B., Liu Z.-K., Wang X.~I., Yang Y.-H., et al., 2022, Natur, 612, 232. doi:10.1038/s41586-022-05403-8

\bibitem[\protect\citeauthoryear{Zemp, Ramirez-Ruiz, \& Diemand}{2009}]{Zemp2009} Zemp M., Ramirez-Ruiz E., Diemand J., 2009, ApJL, 705, L186. doi:10.1088/0004-637X/705/2/L186

\bibitem[\protect\citeauthoryear{Zhang et al.}{2021}]{Zhang2021} Zhang B.-B., Liu Z.-K., Peng Z.-K., Li Y., L{\"u} H.-J., Yang J., Yang Y.-S., et al., 2021, NatAs, 5, 911. doi:10.1038/s41550-021-01395-z


%FBOT discussion

\bibitem[\protect\citeauthoryear{Greiner et al.}{2015}]{Greiner2015} Greiner J., Mazzali P.~A., Kann D.~A., Kr{\"u}hler T., Pian E., Prentice S., Olivares E.~F., et al., 2015, Natur, 523, 189. doi:10.1038/nature14579












==> GRB 210704A/t90.tex <==

{\itshape AGILE}/MCAL&1.06&400-100000& 1\\
{\itshape AstroSat}/CZTI&4.6$^{+2.8}_{-3.6}$&20-200& 2\\
{\itshape Fermi}/GBM &4.7 &50-300& 3 \\
Konus-{\itshape Wind}&4.5&20-4000& 4\\
{\itshape INTEGRAL}/SPI-ACS&$3.5\pm 0.7$&80-1000& 5 \\

